Exponential Lower Bounds for Batch Reinforcement Learning: Batch RL can be Exponentially Harder than Online RL

Several practical applications of reinforcement learning involve an agent learning from past data without the possibility of further exploration. Often these applications require us to 1) identify a near optimal policy or to 2) estimate the value of a target policy. For both tasks we derive \emph{exponential} information-theoretic lower bounds in discounted infinite horizon MDPs with a linear function representation for the action value function even if 1) \emph{realizability} holds, 2) the batch algorithm observes the exact reward and transition \emph{functions}, and 3) the batch algorithm is given the \emph{best} a priori data distribution for the problem class. Our work introduces a new `oracle + batch algorithm' framework to prove lower bounds that hold for every distribution. The work shows an exponential separation between batch and online reinforcement learning.

==> 1-defs.tex <==
%%%%%%%%%%%%%%%%%%% Custom Defs
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{mathtools}
\usepackage{tikz}
\tikzset{>=stealth}
\usetikzlibrary{patterns}
\makeatletter
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{wrapfig}
\usepackage{comment}
\usepackage[export]{adjustbox}
\usepackage{natbib}
\usepackage{subfigure}

\def\wtilde{\widetilde w}
\def\AlgClass{\ensuremath{\mathfrak{B}}}
%\def\Alg{\ensuremath{B}}
\def\Learn{\ensuremath{\mathfrak{L}}}
\def\successor{s^+}
\def\Ca{\overset{\frown}{\mathcal C}}
\def\Ct{\overset{\triangle}{\mathcal C}}
\def\Mpi{\M}
\def\Qpi{Q^{\pi}}
\def\Tpi{\T^\pi}
\def\Mstar{\M^\star}

\def\rdef{
\begin{align}
\text{on} \; M_{w,+}: \quad r_{w,+} (s,a) \defeq \begin{cases}  
0 \quad \quad \quad \text{if} \; a \not \in \C_\gamma(w)\cup \C_\gamma(-w)\\
(1- \gamma)a^\top (+w) \quad \text{otherwise}
\end{cases} \\
\text{on} \; M_{w,-}: \quad r_{w,-} (s,a) \defeq \begin{cases}  
0 \quad \quad \quad \text{if} \; a \not \in \C_\gamma(w)\cup \C_\gamma(-w)\\
(1- \gamma)a^\top (-w) \quad \text{otherwise}
\end{cases} \\
\end{align}
}
\def\Idef{\frac{1}{\gamma} \times \frac{2}{d-1} \times  (1-\gamma^2)^{\frac{d-1}{2}} \times \sqrt{\frac{d}{2\pi}}}
\def\lb{
I^{-1}_{1-\gamma^2}\(\frac{d-1}{2},\frac{1}{2}\)
& \geq \gamma \sqrt{d} \(\(\frac{1}{2}\)\cdot\frac{1}{(1-\gamma)}\)^{\frac{d-1}{2}}, \quad \\
2^{-d}I^{-1}_{1-\gamma^2}\(\frac{d-1}{2},\frac{1}{2}\) & \geq \gamma  \sqrt{d} \(\(\frac{1}{2}\)^{2.5} \cdot \frac{1}{(1-\gamma)}\)^{\frac{d-1}{2}}.
}

==> TexpadSnapshots/2-body_2021-02-04_at_07.45.58.tex <==
\begin{abstract}
%\vspace{-0.4cm}
	Several practical applications of reinforcement learning involve an agent learning from past data without the possibility of further exploration. Often these applications require us to 1) identify a near optimal policy or to 2) estimate the value of a target policy. For both tasks we derive \emph{exponential} information-theoretic lower bounds in discounted infinite horizon MDPs with a linear function representation for the action value function even if 1) realizability holds, 2) the batch algorithm observes the exact reward and transition functions, and 3) the batch algorithm is given the best a priori data distribution for the problem class. Furthermore, if the dataset does not come from policy rollouts then the lower bounds hold even if \emph{all}  policies admit a linear representation. 

If the objective is to find a near-optimal policy, we discover that these hard instances are easily solved by an \emph{online} algorithm, showing that there exist RL problems where \emph{batch RL is exponentially harder than online RL} even under the most favorable batch data distribution. In other words, online exploration is critical to enable sample efficient RL with function approximation. A second corollary is the exponential separation between finite and infinite horizon batch problems under our assumptions.  
On a technical level, this work helps formalize the issue known as \emph{deadly triad} and explains that the \emph{bootstrapping} problem \cite{sutton2018reinforcement} is potentially more severe than the \emph{extrapolation} issue for RL because unlike the latter, bootstrapping cannot be mitigated by adding more samples.
\end{abstract}
\section{Introduction}
While the grand goal of reinforcement learning (RL) is to design fully autonomous agents capable of improving their performance over time by learning from past mistakes, oftentimes a \emph{batch} approach --- which predicts some quantity of interest using past observations only --- is preferable. For example, past data may be available in large quantities and should not be disregarded by adopting a purely online method. In other applications, safety concerns require that the dataset be collected by a carefully monitored procedure, involving a human or a safe controller. In addition, batch algorithms are key tools to build more complex online procedures. These considerations motivate us to investigate whether there exists any \emph{fundamental limitation} to using a batch approach for RL compared to online learning. Concretely, we consider two classical batch reinforcement learning problems: 1) the \emph{off-policy evaluation} (OPE) problem, where the batch algorithm needs to predict the performance of a \emph{target policy} and 2) the \emph{best policy identification} (BPI) problem, where the batch algorithm needs to identify a near optimal policy. 

\paragraph{Linear function approximation} 
As many applications of RL require very large state and action spaces, the hope is that by leveraging strong prior knowledge, for example on the form of the optimal solution, we can learn the critical features of a Markov decision process (MDP) to solve the task at hand without probing the full state-action space. 
For the OPE problem, we assume that the action-value function $\Qpi$ of the target policy $\pi$ can be written at any state action pair $(s,a)$ as an inner product $\phi(s,a)^\top \theta$ between a known feature extractor $\phi$ and an unknown parameter $\theta$ that the learner seeks to identify. For the BPI problem, this representation condition applies to the action-value function $\Qstar$ of an optimal policy.
%Linear methods include representations such as polynomials, Fourier bases, coarse coding, tile coding and radial basis functions \cite{sutton2018reinforcement} and are the building blocks for more complex approximators, such as generalized linear methods and neural networks. 

\paragraph{Quality of the dataset and assumptions}
Batch algorithms are limited by the quality and quantity of the available data: for example, in a tabular MDP, without adeguate coverage of the area of the MDP that the optimal policy tends to visit, there is little hope that we can identify such policy or even predict its performance. However, given enough samples in each state-action pairs,  it becomes easy to identify the optimal policy \cite{Azar12} or to evaluate the value of another \cite{yin2020near}. In addition, without any prior knowledge about the problem or information about the target policy, a uniform distribution over the state-action space is a priori optimal. 

Very recently, some authors have derived exponential lower bounds for the off-policy evaluation problem with linear function approximations \cite{wang2020statistical,amortila2020variant}. They discover that even if a sampling distribution induces the best-conditioned covariance matrix, at least exponentially many samples are needed to estimate the value of a target policy reasonably well. As their hard instances are tabular MDPs (i.e., with small state-action spaces), certainly there exists a better batch distribution: the OPE problem in tabular MDPs is easily solvable by using a uniform distribution over the state-actions coupled with the policy evaluation algorithm on the empirical model. Therefore, their works show that looking at the spectrum of the covariance matrix is not a good test to assess the quality of a batch dataset in RL. This leaves open the question of whether the OPE problem with linear value functions can \emph{always} be solved by using a better dataset of polynomial size (in the horizon and feature dimension), leading to the following question in the context of batch RL with function approximation:
\begin{center}
\textbf{What can a batch algorithm learn using the best a priori distribution for the problem class at hand?}
\end{center}
In particular, we wonder whether  there is any penalty in using an entirely batch approach in place of an online (and adaptive) method if a good dataset is provided to the batch algorithm. To answer this question for both the OPE and BPI problems in the strongest possible way, we consider an auxiliary process or \emph{oracle} that provides the \emph{batch algorithm} with the best data distribution for the task; together they form a \emph{learning algorithm}. However, in contrast to fully online / adaptive algorithms, the oracle is not allowed to change its data acquisition strategy while information is being acquired. As we explain in \cref{sec:MainResult}, this framework allows us to derive strong batch RL lower bounds, because they \emph{will hold for any batch distribution}.

\paragraph{Learning process and assumptions} 
%Precisely, 
We consider oracles that can decide on a set of strategic policies to gather data. 
Alternatively, the oracles can directly specify the state-actions where they want to observe the rewards and transitions (for example, with a simulator). In either case, the oracle selects a sampling strategy and the batch algorithm later receives a \emph{dataset} of states, actions, rewards and transitions. Using the dataset, the batch algorithm makes a prediction, i.e., it  estimates the value of a target policy (OPE problem) or returns a near optimal policy (BPI problem). 
%There exist principled statistical methods that the oracle can use to \emph{find an optimal sampling distribution}; collectively, they are referred to as \emph{design of experiments} \cite{pukelsheim2006optimal} as  they prescribe a distribution (a design) to collect the most informative data (through an experiment). Applications of this powerful theory to linear bandits exist \cite{lattimore2020bandit,wagenmaker2020experimental}. 
We make two other assumptions that favor the learner:
\setlist{nolistsep}
\begin{itemize}[leftmargin=*]
\itemsep0em
\item \emph{Realizability}, 
i.e., there is no misspecification.
\item \emph{Exact feedback}: the exact reward and transition \emph{function} is observed for each point in the dataset. This is equivalent to observing \emph{infinite data} at the selected state-actions.
\end{itemize} 
\vspace{-0.2cm}
\subsection{Contributions}
With such strong assumptions and the freedom of selecting any state-action, identifying a near optimal policy or predicting the value of another should be easy tasks for the learner. For example, in tabular MDPs the oracle could prescribe one query in each state-action pair. This way, the reward and transition functions would become known everywhere, giving  the batch algorithm  complete knowledge of the MDP. For linear bandits with feature vectors spanning $\R^d$, we know that $d$ queries along a basis suffice to identify the full bandit instance. For $H$ horizon MDPs with linear representations, backward induction with $dH$ queries and exact feedback precisely identifies the MDP at hand. 
In all these cases the oracle can find a good sampling distribution for the batch learner, and there is little or no advantage to using an  oracle that adapts the query selection strategy as feedback is received. However, in infinite horizon problems the situation is quite different; we obtain the following \emph{core results}: %there exist problems such that
\setlist{nolistsep}
\begin{enumerate}[leftmargin=*]
\itemsep0em
\item there exists OPE and BPI problems where any batch algorithm must receive an \emph{exponential} $\approx (\frac{1}{1-\gamma})^d$ dataset to return a good answer, 
\item if the dataset does not originate from policy rollouts then the lower bounds hold even if the action-value function of \emph{all policies} admit a linear representation,
\item there exist exponentially hard batch BPI problems (even under the best data distribution) which are easy to solve with online / adaptive algorithms, showing \emph{an exponential separation between batch and online RL},
\item there exist exponentially hard problems for infinite horizon batch RL which cannot arise in finite horizon problems, showing \emph{exponential separation between finite and infinite horizon batch RL}.
\end{enumerate}
Our work also shows that classical globally optimal experimental design yields \emph{provably bad} distributions for infinite horizon RL, making learning impossible even in the limit of infinite data; we discuss this in app. \ref{app:DoE} for space reasons.
%These imply a number of \emph{important consequences}, namely:
%\setlist{nolistsep}
%\begin{enumerate}[leftmargin=*]
%\itemsep0em
%\item there exist exponentially hard problems for infinite horizon batch RL which cannot arise in finite horizon problems, showing \emph{exponential separation between finite and infinite horizon batch RL};
%\item classical globally optimal experimental design yields \emph{provably bad} distributions for infinite horizon RL, making learning impossible even in the limit of infinite data;   we discuss this in \cref{app:DoE} for space reasons.
%\end{enumerate}

We make the following \emph{technical} contributions: % and analytical side:%, we make the following contributions:
\setlist{nolistsep}
\begin{enumerate}[leftmargin=*]
\itemsep0em
\item we present new classes of hard MDP instances where crucial information are hidden in an exponentially small area \emph{of the feature space},
\item we help formalize the hardness induced by the \emph{deadly triad} \cite{sutton2018reinforcement}, i.e., the combination of off-policy learning, bootstrapping and function approximation; in particular, we explain that  \emph{bootstrapping}  is fundamentally different and potentially more severe than the \emph{extrapolation} problem.
\end{enumerate}
\subsection{Literature}
Polynomial lower bounds are often derived to certify that a certain algorithm is sample efficient \cite{jiang2016doubly,duan2020minimax,hao2020sparse}; in this work we are interested in exponential lower bounds. Divergence of dynamic programing algorithms with function approximation is well known \cite{baird1995residual,tsitsiklis1996feature} and has prompted researchers to look for information-theoretic lower bounds for generic predictors \cite{chen2019information} and in presence of misspecification \cite{du2019good}. Concurrently,  \cite{weisz2020exponential,wang2020statistical} also show information-theoretic lower bounds highlighting the danger of \emph{extrapolation} in RL; %however,  their constructions are easily solvable under our assumptions. 
for additional literature, please see \cref{app:Literature}.

\section{Preliminaries}
\label{sec:Defs}
Discounted infinite horizon MDPs \cite{puterman1994markov} are defined by a tuple $M = \langle \StateSpace,\ActionSpace,p,r,\gamma \rangle$, where
$\StateSpace$ is the state space, $\ActionSpace_s$ is the action space in state $s\in\StateSpace$ and $\ActionSpace = \cup_{s\in \StateSpace}\{\ActionSpace_s\} $ is the set of all state-dependent action spaces. We assume that for each state $s \in \StateSpace$ and action $a \in \ActionSpace_s$ there exists a measure $p (\cdot \mid s, a)$ representing the transition dynamics and a scalar reward function $r(s,a) \in [-1,1]$. 
The discount factor $\gamma$ is assumed to be in $(0,1)$. We consider the discounted return of any policy to be $\in [-1,+1]$  (without loss of generality upon rescaling the reward function). 
A deterministic policy $\pi$ maps every state $s\in \StateSpace$ to an action $a\in\ActionSpace_s$. 
The value function of policy $\pi$ in state $s \in \StateSpace$ is defined as $V^\pi(s)= \sum_{t=0}^\infty \gamma^{t}\E_{x_t\sim \pi \mid x_0 = s}r(x_t,\pi(x_t))$;  the limit always exists and it is finite under our assumptions as long as the expectation is well defined. The action-value function $Q^\pi$ of policy $\pi$ in $(s,a)$ also exists and is defined as $Q^\pi(s,a)= r(s,a) + \sum_{t=1}^\infty \gamma^{t}\E_{x_t\sim \pi \mid (s,a)}r(x_t,\pi(x_t))$.
An optimal policy $\pistar$, when it exists, is defined in every state as $\pistar(s) = \argmax_\pi V^\pi(s)$ and the corresponding value function and action-value function are denoted  with $\Vstar = V^{\pistar}$ and $\Qstar = Q^{\pistar}$. We sometime add the subscript $M$ to indicate that a certain quantity depends on the MDP $M$ under consideration (e.g., we write $\Vstar_M$). The Euclidean ball in $\R^d$ is defined as $\B = \{ x\in\R^d \mid \| x \|_2 \leq 1 \}$.
The \emph{Bellman optimality operator} $\T$ and the \emph{Bellman evaluation operator} $\T^\pi$ are mappings between action value functions: % defined as
\vspace{-0.1cm}
\begin{align*}
(\T Q)(s,a) & = r(s,a) + \gamma\E_{s' \sim p(s,a)} \sup_{a' \in \ActionSpace_{s'}}Q(s',a') \\ 
(\T^{\pi} Q)(s,a) & = r(s,a) + \gamma\E_{s' \sim p(s,a)} Q(s',\pi(s')).
\end{align*}
\vspace{-1cm}
\section{Batch Reinforcement Learning}
We first formally define the two  \emph{learning problems}, namely the task of returning a near optimal policy, also known as \emph{best policy identification} (BPI) problem, and the task of predicting the value of a \emph{target policy}, also known as \emph{off-policy evaluation} (OPE) problem. Then, in the next four sub-sections we describe the learning process in more detail. The lower bounds that we later derive will hold for all algorithms of the form described in this section.

A \emph{BPI problem} $(s^\star,\{ M \in \M\} )$ is defined by a starting state $s^\star$ and a class $\M$ of MDPs sharing the same state space, action space and discount factor. 
An \emph{OPE problem} $(s^\star,\{(M,\pi_M) \mid M \in \M\})$ additionally requires us to identify one or more target policies
$\pi_M$ for each $M \in \M$. 

Depending on the problem, the oracle selects a sampling strategy such that for every \emph{problem instance} $(s^\star,M,\pi_M)$ (of an OPE problem) or $(s^\star,M)$ (of a BPI problem) the batch algorithm  experiences a dataset $\mathcal D$ from $M$ and uses it to return an accurate estimate $\Qhat_{\mathcal D}$ of the action-value function of $\pi_M$ at $s^\star$ (for the OPE problem) or a near optimal policy $ \pihatstar_{\mathcal D}$ on $M$ from $s^\star$ (for the BPI problem).
\begin{minipage}{0.49\textwidth}
\begin{algorithm}[H]
\footnotesize
\floatname{algorithm}{Protocol}
\begin{algorithmic}[1]
\caption{\footnotesize \textsc{Batch RL with a Strategic Oracle}}
\label{alg:Policy:BatchLearner}
\STATE \emph{(Input)} Oracle receives a batch problem and budget $n$
\STATE \emph{(Query Selection)} Oracle chooses $\mu$ (def. \ref{asm:PolicyFree})
or $T$ (def. \ref{asm:PolicyInduced}).
\STATE \emph{(Data Collection)} Batch algorithm receives the dataset $\mathcal D$% = \{(s,a,r(s,a),p(s,a)) \mid \forall (s,a) \in \mu\}$ 
\STATE \emph{(Output)} Batch algorithm returns $\Qhat_{\mathcal D}$ or $\pihatstar_{\mathcal D}$ %depending on the learning goal
\normalsize
\end{algorithmic}
\end{algorithm}
\end{minipage}
\subsection{Step I: Input}
\label{sec:step1}
The oracle receives \emph{either} an OPE or a BPI problem together with a \emph{query budget} $n\in \mathbb N$. The oracle has access to each instance of the problem it is given, and in particular it knows the state and action spaces $\StateSpace,\ActionSpace$, the discount factor $\gamma$, and the full set of transition functions and reward functions for each MDP $M\in\M$, but it does not know which of these MDPs in $\M$ it will interact with or what the target policy will be. In addition, the oracle has full knowledge of the batch algorithm.

\subsection{Step II: Query Selection}
\label{sec:step2} 
The purpose of the oracle is to help the batch algorithm by providing it with the best dataset for the specific problem at hand. 
To capture different mechanisms of data acquisition, we consider two methods to specify the \emph{query set}, i.e., the set of state-action pairs where the oracle wants the batch algorithm to observe the rewards and the transitions. In the first mechanism the oracle directly selects the state-actions; we place no restriction on the mechanism to obtain these queries as long as the sampling distribution is fixed for all MDPs in the class.
\begin{definition}[Policy-Free Queries]
\label{asm:PolicyFree} 
A set $\mu$ of state-action pairs is said to be policy-free for an OPE or BPI problem if $\mu$ does not depend on the specific MDP instance $M \in \M$.
\end{definition}
The second mechanism to collect data is by selecting deterministic\footnote{This is not a restriction: for any given stochastic policy the agent can sample an action from the distribution of actions in every state before deploying the policy.} policies. The policies will generate random trajectories that the batch algorithm later observes. Since we are interested in what the agent can learn in the limit of infinite data (i.e., under exact feedback) we let the batch algorithm observe \emph{all possible realizations} of such trajectories. With this aim, we define the state-action space reachable in $c$ or less timesteps from $s_0$ using policy $\pi$ as $\Reach(s_0,\pi,c) = $
\begin{align*}
\{(s,a) \mid \exists t < c, \; \text{s.t.} \; \Pro\( (s_t,a_t) = (s,a) \mid \pi,s_0 \) > 0  \}
\end{align*}  
where $(s_t,a_t)$ is the random  state-action encountered at timestep $t$ upon following $\pi$ from $s_0$.
We let the oracle select the best combination of trajectory lengths and number of distinct policies.

\begin{definition}[Policy-Induced Queries]
\label{asm:PolicyInduced}
Consider an OPE or BPI problem and fix a set $T = \{ (s_{0i},\pi_i,c_i) \}_{i=1}^\kappa$ of triplets, each containing a starting state $s_{0i}$, a deterministic policy $\pi_i$ and a trajectory length $c_i$ such that $\sum_{i=1}^\kappa c_i \leq n$. 
Then the query set $\mu$ induced by $T$ is defined as
\begin{align*}
\mu \defeq \bigcup_{(s_{0},\pi,c) \in T} \Reach(s_{0},\pi,c).
\end{align*}
\end{definition} 
\vspace{-0.4cm}
The condition $\sum_{i=1}^\kappa c_i \leq n$ attempts to make the amount of information acquired using policy-free queries comparable to the policy-induced query method, although the latter generates $|\mu| \geq n$ if the dynamics are stochastic. In other words, the batch learner always observes at least $n$ state-actions if these are induced by policies.

\begin{remark}
\label{rem:PolicyInducedIsPolicyFree}
A policy-induced query set is also policy-free whenever the dynamics of each MDP $M\in\M$ are the same. 
\end{remark} 

\begin{remark}
	When prescribing a set $T$ the oracle has knowledge of the induced dataset $\mu$ for each choice of $T$ (e.g., by having access to a connectivity graph of the MDP).
\end{remark}

While a policy-free query set may seem less constrained than a policy-induced query set, the latter may implicitly reveal additional information about the dynamics of the MDP whenever the induced trajectories are all different across different MDPs.

\subsection{Step III: Data Collection}
After the oracle has submitted the sampling strategy, the batch learner receives a dataset $\mathcal D$ which contains the \emph{exact} reward and transition \emph{function}, $r(s,a)$ and $p(s,a)$, from the MDP $M \in \M$ for each $(s,a)$ in the query set $\mu$. 
\subsection{Step IV: Output}
\label{sec:step4}
The batch algorithm is finally required to make a prediction using the acquired dataset $\mathcal D$. For the OPE problem, the batch algorithm also receives the target policy $\pi_M$ and it is required to output an estimator $\Qhat_{\mathcal D}$ for the action-value function of the target policy $Q_M^{\pi_M}(s^\star,\cdot)$; for the BPI problem, it must output a near-optimal policy $\pihatstar_{\mathcal D}$ at $s^\star$.

\subsection{Evaluation Criterion}
\label{sec:evaluation}
The \emph{oracle} and the \emph{batch algorithm} together form a \emph{learning algorithm}. This framework allows us to derive batch lower bounds in a strong form as they will hold for any data distribution. We say that the learning algorithm is \emph{$(\epsilon,\delta)$-sound} for an OPE problem
if for every instance 
$(s^\star,M,\pi_M)$ of the problem the returned estimator $\widehat Q_{\mathcal D}$ is accurate w.h.p.:
$$\Pro\( \sup_{a\in \ActionSpace_{s^\star}}|(Q_M^{\pi_M} - \Qhat_{\mathcal D})(s^\star,\cdot) | < \epsilon \) > 1-\delta. $$
Similarly, we say that that the learning algorithm is \emph{$(\epsilon,\delta)$-sound} for a BPI problem if for every instance $(s^\star,M)$  it holds that the returned policy $\pihatstar_{\mathcal D}$ is near optimal w.h.p.:
$$\Pro\( (\Vstar_M - V_M^{\pihatstar_{\mathcal D}})(s^\star)  < \epsilon \) > 1-\delta.$$
As the query set is always non-random and the batch algorithm experiences the exact reward and transition function, the only  randomness lies in the possible randomization internal to the batch algorithm when it returns an answer.

\subsection{Adaptive and Online Algorithms}
Consider a policy-free mechanism. We say that a learning algorithm is \emph{adaptive} if every time the oracle  submits a state-action it receives the feedback from the environment and can use it to select the next state-action to query the MDP.

Likewise, consider a policy-induced mechanism. We say that a learning algorithm is acting \emph{online} if every time the oracle selects a policy and trajectory length, it can use the acquired feedback to  select the next combination of policy and trajectory length (its position is reset in every episode).
%\vspace{-0.3cm}
\section{Intuition}
\begin{figure*}[t!]
\vspace{-0.6cm}
\centering    
\begin{adjustbox}{minipage=\linewidth,scale=1.0}
\subfigure{
\label{fig:DoE}
\input{fig1.tex}}
\subfigure{\label{fig:Multiple}
\input{fig2.tex}}
\hspace{-2mm}
\subfigure{
\label{fig:Cap}
\input{fig3.tex}}
\hspace{-0mm}
\begin{minipage}[b]{0.35\linewidth}
\caption{ 
\emph{Left}: the orthogonal blue vectors $\phi_1,\phi_2$ represent the choice of the algorithm, while $\phi^+_1,\phi^+_2$ are the corresponding successor features. The learner thus acquires information only along the vertical direction.
\emph{Middle}: in the figure $\mathcal R = \Range(\Phi^\top-\gamma(\Phi^+)^\top)$ and $\mathcal N = \Null(\Phi-\gamma\Phi^+)$. 
\emph{Right}: in this case the next-state discounted feature $\gamma\phi^+_i$ cannot project $\phi_i$ onto the vertical plane because of the discount factor $\gamma < 1$.}
\end{minipage}
\end{adjustbox}
\vspace{-0.6cm}
\end{figure*}
The mechanism that induces hardness for infinite horizon problems must be different than that in finite horizon: the constructions from \cite{weisz2020exponential,wang2020provably} rely on the \emph{extrapolation} issue that compounds the errors multiplicatively. In our case, the reward and transition functions are observed exactly, so there is no error to extrapolate in the first place. Instead, \emph{bootstrapping} is the root cause of hardness; we provide some intuition in this section. 

While all theorems necessitates of a different construction, they all build on the intuition presented in this section. At a high level, using function approximation the agent hopes to make predictions on unseen state-actions. Unfortunately, bootstrapping can ``erase'' the information gained along certain directions in feature space, but an off-policy prediction problem can require the agent to make predictions precisely along those directions where information are missing.

Suppose that the oracle is trying to find a good policy-free query set for the off-policy problem on a class of MDPs with feature vectors $\phi(\cdot,\cdot)$ anywhere in the unit Euclidean ball. % $\B \subseteq \R^d$. 
Denote with $(s_1,a_1),\dots,(s_n,a_n)$ the state-actions chosen by the oracle and with $(s^+_1,a^+_1),\dots,(s^+_n,a^+_n)$ the corresponding successor states and actions\footnote{Assume deterministic successor states; the actions in the successor states are determined by the target policy (OPE problem) or by an $\argmax$ function (BPI problem).}.
Intuitively, choosing a set $\phi(s_1,a_1), \dots, \phi(s_n,a_n)$ of orthogonal feature vectors of maximal length seems to be the best the oracle can do. In \cref{fig:DoE} we represent the feature space of an RL problem where the learner can choose any feature vector in the Euclidean ball in $\R^2$; the agent's choice of the feature $\phi_i=\phi(s_i,a_i)$ would indeed be a a choice arising from globally optimal experimental design. 
Define
\begin{align*}
\hspace{-2mm}
%\label{main:eq:Phi}
\Phi = \begin{bmatrix}
\phi(s_1,a_1)^\top \\
\dots \\
\phi(s_n,a_n)^\top
\end{bmatrix},
r = \begin{bmatrix}
r(s_1,a_1) \\
\dots \\
r(s_n,a_n) 
\end{bmatrix},  
\Phi^+ = \begin{bmatrix}
\phi(s^+_1,a^+_1)^\top \\
\dots \\
\phi(s^+_n,a^+_n)^\top
\end{bmatrix}
\end{align*}

After observing the reward and successor states, we can write down the local (i.e., at the state-actions chosen by the oracle) Bellman equations. If we leverage the known functional form of the action-value function of the target policy we can write the following linear system, whose solution (in terms of $\theta \in \R^d$ or action-value function $\Phi\theta$) the batch algorithm seeks to discover:
\begin{align}
\label{eqn:FinalLinearSystem}
\Phi\theta = r + \gamma\Phi^+\theta \quad \longrightarrow \quad  (\Phi -\gamma\Phi^+)\theta = r
\end{align}
Unlike machine learning or bandit problems where the agent directly observes a response from $\phi(s_i,a_i)$,  bootstrapping the future returns makes the agent observe a response (i.e., the reward) corresponding not to $\phi(s_i,a_i)$ but to  $\phi(s_i,a_i) - \gamma \phi(s^+_i,a^+_i)$, which we call ``effective feature vector'', see \cref{eqn:FinalLinearSystem}. 
Unfortunately, $\phi(s^+_i,a^+_i)$ can act adversarially. As an example, consider \cref{fig:DoE} in $\R^2$ where the orthogonal feature vectors chosen by the agent are projected along the vertical direction by bootstrapping: the net effect is that the agent only learns along one axis.

Unfortunately, choosing more feature vectors does not easily solve the problem as the next state discounted feature vector can ``erase'' what the agent learns in one direction of the feature space (\cref{fig:Multiple}). To acquire information in all directions (i.e., to ensure a non-singular $\Phi - \gamma\Phi^+$ in \cref{eqn:FinalLinearSystem})  the oracle must probes the small spherical cap in \cref{fig:Cap}. Which spherical cap to probe is unknown ahead of sampling (as the target policy or the optimal policy are unknown), and thus the oracle needs to probe all of them if it wants the batch algorithm to confidently solve the problem. Using the fact that there are exponentially many spherical caps in an Euclidean ball in $\R^d$, we conclude.

\paragraph{Exponential separation with online learning}
An online algorithm can detect that the next-state feature matrix $\Phi^+$ is acting adversarially. In addition, $\Phi^+$ encodes the location of the spherical cap in \cref{fig:Cap}. Probing the spherical cap reveals crucial information about the MDP, and in particular it makes the linear system in \cref{eqn:FinalLinearSystem} full rank.
%In this example, the next-state feature matrix $\Phi^+$ is constr adversarially

\section{Exponential Lower Bounds}
\label{sec:MainResult}
We define the \emph{query complexity to $(\epsilon,\delta)$-soundness of a problem} (OPE or BPI) to be the minimum value for $n$ (as in \cref{asm:PolicyFree,asm:PolicyInduced}) such that there exists a $(\epsilon,\delta)$-sound learning algorithm for that problem. In particular, the query complexity depends on the MDP class $\M$ and can be different for the OPE and BPI tasks and for the policy-free and policy-induced query mechanism. 

The lower bounds %that we present 
are expressed in terms of the regularized incomplete beta function $I_x(a,b) = B(x,a,b)/B(1,a,b)$ where $B(x,a,b)$ is the incomplete beta function for some positive real numbers $a,b$ and $x \in [0,1]$; for the precise definitions, please see \cref{app:additional_notation}. Let $
	\mathcal N(\gamma,d) = I^{-1}_{1-\gamma^2}\(\frac{d-1}{2},\frac{1}{2}\)
$ for short; \cref{cor:LowerBound} for $d \geq 5$ ensures
\begin{align*}
\mathcal N(\gamma,d) \geq 2^{-d}\mathcal N(\gamma,d) & \geq \gamma  \sqrt{d} \( \frac{1}{2^{2.5}(1-\gamma)} \)^{\frac{d-1}{2}} \approx \(\frac{1}{1-\gamma}\)^d.
\end{align*}
\subsection{Realizability Assumptions}
Unless additional assumptions are made regarding the MDP class $\M$ that defines the OPE and BPI problems, the query complexity of a reasonably sound  learner is exactly the size of the state and action space (we assume exact feedback). One hopes that by restricting the MDP class $\M$, the query complexity of the OPE and BPI problems can be brought down to a more manageable level, in particular, independent of the state-action spaces.

We make one of the following three assumptions (only one assumption will hold at any given time, depending on the theorem); two are known as realizability, and the third is strictly stronger than the first two. The first concerns the OPE problem.

\begin{assumption}[$Q^\pi$ is Realizable]
\label{asm:OPE:MDP}
Given an OPE problem $(s^\star,\{(M,\pi_M), M\in\M\})$, there exists a $d$-dimensional map $\phi(\cdot,\cdot)$ such that $\|\phi(\cdot,\cdot)\|_2 \leq 1$ and for any  $M\in \M$ the action-value function of the target policy $\pi_M$ satisfies $\forall (s,a), Q_M^{\pi_M}(s,a) = \phi(s,a)^\top \theta_M$ for some $\theta_M \in \B$.
\end{assumption}
For the BPI problem the representation condition applies to the action-value function  of an optimal policy.

\begin{assumption}[$\Qstar$ is Realizable]
\label{asm:BPI:MDP}
Given a BPI problem $(s^\star,\{M\in\M\})$, there exists a $d$-dimensional feature map $\phi(\cdot,\cdot)$ such that $\|\phi(\cdot,\cdot)\|_2 \leq 1$ and for any  $M\in \M$ there exists $\theta_M^\star\in \B$ such that the optimal action-value function is linear: $\forall (s,a), \Qstar_M(s,a) = \phi(s,a)^\top \theta_M^\star$.
\end{assumption}

A stronger assumption we make is that \emph{all} policies are linearly representable.

\begin{assumption}[$Q^\pi$ is Realizable for all Policies]
\label{asm:ALL:MDP}
Given a BPI problem $(s^\star,\{M\in\M\})$ or an OPE problem $(s^\star,\{(M,\pi_M), M\in\M\})$, there exists a $d$-dimensional feature map $\phi(\cdot,\cdot)$ such that $\|\phi(\cdot,\cdot)\|_2 \leq 1$ and for any MDP $M\in\M$ the value of any policy $\pi$ satisfies $\forall (s,a), Q_M^{\pi}(s,a) = \phi(s,a)^\top \theta^{\pi}_M$ for some $\theta^{\pi}_M \in \B$.
\end{assumption}

The learners that we consider are aware of these assumptions because they can examine each MDP in the class $\M$ they receive (see \cref{sec:step1}).

\subsection{Off-Policy Evaluation} %and Strong Form}
 
The first result of this work is contained in the following lower bound for the OPE problem; since all MDPs in $\M$ share the same dynamics, the oracle has full knowledge of the actions it needs to take to visit any state-action it desires.  %The construction  uses a class of \emph{stateless} MDPs, i.e., MDPs where the state has no effect on the rewards and on  the (deterministic) transitions.
\begin{theorem}[OPE Policy-Induced Lower Bound]
\label{thm:OPE:Policy-Induced}
There exists an OPE problem $(s^\star,\{(M,\pi_M), M\in\M\})$  satisfying \cref{asm:OPE:MDP} such that its policy-induced query complexity to $(1,1/2)$-soundness  is at least $
\mathcal N(\gamma,d)$. 
\end{theorem}

%We mention that if the target policy is known, there exists an online algorithm for this OPE problem that can identify $Q^{\pi_M}_M(s^\star,\cdot)$ with probability one by playing one specific action in the start state $s^\star$.

%If the oracle is acting online but has no knowledge of the target policy then an essentially equivalent lower bound can be obtained. In either case, 

It is useful to compare the \emph{form} of the above lower bound with that of some concurrent results for the off-policy evaluation problem: for example, \cite{wang2020statistical,amortila2020variant}  show that \emph{there exist} a sampling distribution $\mu$ (that induces the best-conditioned covariance matrix), a target policy $\pi$ and an MDP class $\widetilde \M$, each satisfying certain properties, such that the best estimator on the most difficult MDP in $\widetilde \M$ performs poorly if less than exponentially many  samples are used. However, in their case there exists a better batch distribution of polynomial size that solves the problem. 
Our instances are instead much harder, as they command an exponential dataset even for the \emph{best} distribution for the task: since the oracle can prescribe any data distribution, we can claim that \emph{for all} distributions of polynomial size we can find an MDP subclass $\widetilde \M \subseteq \M$ and a target policy such that all MDPs in $\widetilde \M$ generate similar datasets but the value of the target policy is very different on these MDPs in $\widetilde \M$, giving lower bounds in a \emph{stronger form}.
 
\subsection{Best Policy Identification}% Lower Bound and Exponential Separation}
As in \cref{thm:OPE:Policy-Induced}, in the next lower bound the oracle knows the set $\mu$ induced by any choice of $T$ (see \cref{asm:PolicyInduced}).
\begin{theorem}[BPI Policy-Induced Lower Bound]
\label{thm:BPI:Policy-Induced}
There exists a BPI problem $(s^\star,\{M\in\M\})$ satisfying \cref{asm:BPI:MDP} with features in dimension $d+1$ such that its policy-induced query complexity to $(1/2,1/2)$-soundness is at least $ 
2^{-d}\mathcal N(\gamma,d)$.
\end{theorem} 
Hard BPI problems for adaptive and online algorithms are given by \citet{weisz2020exponential}. Clearly, their construction can be embedded in an infinite horizon MDP, giving a lower bound under their assumptions. However, our framework allows the learner to observe the \emph{exact} reward and transition function, which is equivalent to having infinite data at the selected state-actions. In such case, the construction of \citet{weisz2020exponential} no longer gives rise to hard instances. In particular, the BPI problem with our assumptions becomes straightforward in finite horizon, showing an exponential separation between finite and infinite horizon batch RL.

\subsection{Exponential Separation to Online Learning}
\begin{theorem}[Exponential Separation to Online Learning]
\label{thm:BPI:ExponentialSeparation}
Consider the same BPI problem as in \cref{thm:BPI:Policy-Induced}. There exists an  online algorithm that can identify an optimal policy with probability one by observing trajectories of length one with exact feedback from $d+1$ distinct policies from $s^\star$.
\end{theorem} 
 This result shows \emph{exponential separation with online learning} even when the best batch distribution is used. Key information are hidden in an exponentially small area of the feature space whose position is a priori unknown. However, an online algorithm can learn where these information are hidden and then probe such region as we show in \cref{main:sec:Proof}.

\subsection{Lower Bounds with Stronger Representations}

We now wonder what is achievable if the oracle can specify the queries anywhere in the state-action space without the restriction imposed by following policies (i.e., by specifying a policy-free query set). Under this assumption the situation gets surprisingly worse, as the lower bounds now hold even if the action-value function of \emph{all} policies is linearly representable. The explanation is that if the dataset does not come from policy rollouts then the batch algorithm does not observe important information about the dynamics, giving rise to harder problem classes. %Surprisingly, the target policy for the OPE problem below is fixed across all MDPs, and thus \emph{it is  known to the oracle}. 

\begin{theorem}[Policy-Free Lower Bounds]
\label{thm:ALL:Policy-Free}
There exist an OPE problem $(s^\star,\{(M,\pi_M), M\in\M\})$ and a BPI problem $(s^\star,\{M\in\M\})$, which satisfy \cref{asm:ALL:MDP} and share the same $s^\star$ and $\M$, such that their policy-free query complexity to $(1,1/2)$-soundness is at least $
\mathcal N(\gamma,d)$. %For the same OPE and BPI problems, there exist both an adaptive strategy and an online algorithm that can identify $Q^{\pi_M}_M(s^\star,\cdot)$ and the optimal policy with probability one using at most $d+1$ policy-free queries (for the adaptive algorithm) or $d+1$ trajectories of length one (for the online algorithm).
\end{theorem}
\vspace{-0.1cm}
If policy rollouts were allowed then the policy iteration algorithm \cite{lagoudakis2003least} or algorithms based on policy gradient \cite{agarwal2020optimality} would easily find a near optimal policy \emph{for any problem} that satisfies \cref{asm:ALL:MDP}. However, these methods need to interact with the environment to proceed, i.e., they are non-batch. Our result thus shows that it is not possible to start from a batch dataset obtained from a generative model and a run these algorithms successfully without acquiring further data, even if a  strong representation holds.

%For the BPI problem, the exponential separation with online RL is even more surprising in \cref{thm:ALL:Policy-Free}: while the oracle can select any state-action (or feature vector) it desires through a generative model, an online algorithm needs to navigate the unknown environment to acquire such information, and most importantly, how to navigate the environment is not necessarily encoded in the function approximator associated to the problem.

Contrasting \cref{thm:ALL:Policy-Free} with \cref{thm:OPE:Policy-Induced,thm:BPI:Policy-Induced} shows that there is a sharp distinction in what can be achieved depending on the \emph{mechanism} that generates the dataset, a distinction which is absent in tabular RL.
\vspace{-0.2cm}
\section{Proof Sketch}
\label{main:sec:Proof}
%\begin{figure*}[t!]
%\centering    
%\begin{adjustbox}{minipage=\linewidth,scale=1.0}
%\subfigure{\input{fig4.tex}}
%\begin{minipage}[b]{0.35\linewidth}
%\caption{}
%\end{minipage}
%\end{adjustbox}
%\end{figure*}
We now highlight the steps needed to prove \cref{thm:BPI:Policy-Induced} and \cref{thm:BPI:ExponentialSeparation}. After describing the MDP and verifying realizability, both results can be proved in few lines. 
\vspace{-0.1cm}
\subsection{MDP Class}
We consider a class $\M$ of MDPs sharing the same state-space $\mathcal S$, action space $\ActionSpace$ and discount factor $\gamma > 0$, but different transition function $p$ and reward function $r$. We first describe the state and action space which are fixed across all MDPs in the class $\M$. 

At a high level, each MDP contains a two-armed bandit instance in $s^\star$ (the starting state). There, the learner has two choices: either take the special action $a^\star$ that leads to the terminal state $s^\dagger$ and gives an immediate reward of $\frac{1}{2}$, or take any other action that leads to the positive orthant $\mathcal B^+ = \{x\in\R^d  \mid x_i \geq 0, i \in [d]\}$ where the maximum return is either zero or one (depending on the sign $\pm$) but is hidden in an exponentially small region, see \cref{fig:Quarter}. As the learner is unable to discover the maximum return inside $\mathcal B^+$, it does not know if $a^\star$ is the optimal action in $s^\star$. 
\paragraph{State space}
The state space $\StateSpace$ can written as a disjoint union of the positive orthant with the starting state $s^\star$ and terminal state $s^\dagger$:
 $
\StateSpace = \B^+ \uplus \{s^\star\} \uplus \{ s^\dagger \}.
$
\paragraph{Action space}
In the starting state $s^\star$ a special action $a^\star$ is available in addition to any action in $a \in \B^+$, i.e., the actions can be represented as vectors in $\mathcal B^+$. Otherwise, for states in $\B^+$, any action in $\B^+$ is available. Finally, in the terminal state $s^\dagger$ only $\vec 0 \in \B^+$ is available. Mathematically:
%\vspace{-0.7cm}
\begin{align*}
\ActionSpace_s \defeq \begin{cases}
\B^+ \cup \{ a^\star \}  & \text{if} \; s = s^\star \\
\B^+ & \text{if} \; s \in \B^+  \\
\{\vec 0\}  & \text{if} \; s = s^\dagger.
\end{cases}
\end{align*}
%\textbf{Discount factor}:
%The discount factor $\gamma \in (0,1)$. \\
%\textbf{Feature map}:
%The feature map is defined as follows
%\begin{align*}
%\phi(s,a) = 
%\begin{cases}
%[a,0] & \text{if}\; a\in \B^+ \\
%[\vec 0,1] & \text{if}\; a = a^\star \quad \text{(only available in $s^\star$).}
%\end{cases}
%\end{align*}
\vspace{-0.7cm}
\subsection{Instance of the class}
\begin{figure}[b]
\centering  
\hspace{-0.7cm}
\subfigure{\input{fig4.tex}}
\begin{minipage}[b]{0.54\linewidth}
\caption{State space and possible outcomes upon taking the state-action $(s^\star,a_1)$ and then $(a_1,a_2)$. Both $M_{w,+}$ and $M_{w,-}$ have identical reward and transition functions outside the dark gray area.}
\label{fig:Quarter}
\end{minipage}
\vspace{-1.0cm}
\end{figure}
%Next we describe the MDP-specific transition and reward functions. 
Every MDP $M \in \M$ is identified by a vector $w \in \partial\B^+$  and by a $+$ or $-$ sign, and is denoted with $M_{w,+}$ or $M_{w,-}$. %, respectively.\\
\paragraph{Transition function}:
The transition function depends on the vector $w$ that identifies each MDP in the class, but not on the sign $+$ or $-$. Fix the MDP by fixing $w$ (two MDPs correspond to a given choice of $w$). If the agent plays the special action $a^\star$, which is only available in the starting state $s^\star$, it transitions with probability one to the terminal state $s^\dagger$. If the agent plays $a \neq a^\star$, the transition function only depends on the action $a$ (and not on the current state $s$) and the successor state coincides with the action taken with some probability, and is otherwise the absorbing state $s^\dagger$.  

Mathematically, if $a = a^\star$ then $p_w(s' = s^\dagger \mid (s^\star,a^\star)) = 
1$ and if conversely $a \in \B^+$:
\begin{align*}
\begin{cases}
	p_w(a \mid s,a) & = 
\min\{ (1/\gamma) a^\top w, 1 \}, \\ p_w( s^\dagger \mid s,a) & = 1 - p_w(a \mid s,a),
\end{cases}
\end{align*} 
and particular, the definition implies that the successor state is always either $a\in\B^+$ or the terminal state $s^\dagger$.
%\begin{align*}
%p_w(s' \not \in \{ a,s^\dagger\} \mid (s,a)) & = 0.
%\end{align*}
\paragraph{Reward function}
The reward function depends on both the vector $w \in \partial\B^+$ and on the sign $+$ or $-$ that identifyies the MDP. It is always $\frac{1}{2}$ if the special action $a^\star$ is taken and otherwise it is everywhere $0$ on $M_{w,-}$ or is positive only in the hyperspherical cap on $M_{w,+}$. Mathematically $\forall (s,a)$:
\begin{align*}
\text{on} \; M_{w,+}& , \quad r_{w,+}(s,a) \defeq \begin{cases} 
\frac{1}{2}\; \; \; \text{if} \; (s,a) = (s^\star,a^\star)\\
\max\{a^\top w - \gamma, 0 \} \; \text{otherwise,} \;
\end{cases} \\
\text{on} \; M_{w,-}& , \quad r_{w,-}(s,a) \defeq \begin{cases} 
\frac{1}{2} & \text{if} \; (s,a) = (s^\star,a^\star)\\
0 & \text{otherwise.} \;
\end{cases}
\end{align*}
%\textbf{Optimal action-value function}: 
%$M_{w,+}$ and $M_{w,-}$ \emph{have identical transition functions but different reward functions}. %In particular, in both $M_{w,+}$ and $M_{w,-}$ the reward function is everywhere zero except on the small hyperspherical cap \info{...}.
Each MDP in the class has a linear $\Qstar$ function.% function of the vector $w$ and the sign $\pm$.

\begin{lemma}[$Q^\star$ is Realizable; \cref{lem:BPI:Policy:Realizability} in appendix]
\label{main:lem:BPI:Policy:Realizability} Let $\Qstar_{w,+}$ and $\Qstar_{w,-}$ be the optimal $\Qstar$ values on $M_{w,+}$ and $M_{w,-}$, respectively. There exists a feature extractor $\phi: \StateSpace\times \ActionSpace \rightarrow \R^d$ such that for any $w\in\partial\B^+$ it holds that
\begin{align*}
%\label{eqn:BPI:Policy:Solution}
\forall (s,a), \quad \begin{cases}
\Qstar_{w,+}(s,a) = \phi(s,a)^\top [w,\frac{1}{2}] \quad \text{on} \; M_{w,+},\\
\Qstar_{w,-}(s,a) = \phi(s,a)^\top [\vec{0},\frac{1}{2}] \quad \text{on} \; M_{w,-}.
\end{cases}
\end{align*}
\vspace{-0.5cm}
\end{lemma}
\subsection{Proof Sketch of Theorem \ref{thm:BPI:Policy-Induced}}
Define the spherical cap $
\C_\gamma(w) = \{ \| x\|_2 \leq 1 \mid \frac{x^\top w}{\|w\|_2} \geq \gamma \}
$.
The steps for the proof are the following: 1) by construction, policy-induced queries are also policy-free 2) using less than exponentially many samples ensures that at least one spherical cap $\mathcal C_\gamma(\wtilde)$ is not probed 3) the corresponding $M_{\wtilde,+}$ and $M_{\wtilde,-}$ look the same outside the spherical cap $\mathcal C_\gamma(\wtilde)$ and 4) the agent has thus not enough information to distinguish $M_{\wtilde,+}$ from $M_{\wtilde,-}$.
\paragraph{Policy-free vs policy-induced queries}
Notice that although the dynamics are different for different $w$'s (that identify the MDP), any set $T$ (\cref{asm:PolicyInduced}) induces the same set $\mu$ of state-actions (possibly with the exception of $(s^\star,a^\star)$ and $ (s^\dagger,\vec 0)$) regardless of the vector $w$ and the sign $\pm$. We can therefore consider the case that the oracle has chosen a policy-free query set $\mu = \{(s_i,a_i)\}_{i=1}^{n} \cup \{(s^\star,a^\star), (s^\dagger,\vec 0)\}$. %, where the stat-actionpairs are the possible state-actions visited by the behavioral policies chosen by the oracle. 
\paragraph{Existence of exponentially many hyperspherical caps}
We have the following result where we define the outer portion of the positive orthant $\partial \B^+=\{x\in \partial\B \mid \|x \|_2=1 \}$.
\begin{lemma}(Follows from \cref{lem:LonelyPlus} in appendix)
Assume that less than $2^{-d}\mathcal N(\gamma,d)$ actions $a_1,\dots,a_n$ on $\mathcal B^+$ are tried. Then there exists a spherical cap $\C_\gamma(\wtilde)$ that no action has probed, i.e., $\forall i\in[n], a_i \not \in \C_\gamma(\wtilde)$.
	%For any set of vectors $\{a_i\}_{i=1}^n, a_i \in \mathcal B^+$, if $n < \mathcal N(\gamma,d)$ then $\exists \wtilde \in \partial\B^{+}$ such that  $\forall i\in[n], a_i \not \in \C_\gamma(\wtilde)$.
\end{lemma}
%The lemma says that if less than exponentially many actions on $\mathcal B^+$ are tried, then there exists a spherical cap $\C_\gamma(\wtilde)$ that no action $a_1,\dots,a_n$ has probed; 
In this case, the agent does not have any information originating from inside the dark gray hyperspherical cap in \cref{fig:Quarter}. %which contains critical information about the MDP sign $\pm$. 

\paragraph{Outside of the hyperspherical cap $\boldsymbol {M_{w,+} = M_{w,-}}$}
Unfortunately $M_{w,+}$ and $M_{w,-}$ look identical outside of the hyperspherical cap. Precisely, if $n < \mathcal N(\gamma,d)$, consider $\wtilde$ given by the above lemma and the two associated MDPs $M_{\wtilde,+}$ and $M_{\wtilde,-}$.  Notice that the transition function is by construction identical on $M_{\wtilde,+}$ and $M_{\wtilde,-}$ while their reward function is zero at any state action selected by the oracle: $\forall (s,a)\in \{(s_i,a_i) \}_{i=1}^n$ it holds that
\begin{align*}
r_{\wtilde,+}(s,a) = r_{\wtilde,-}(s,a) \quad \text{and} \quad p_{\wtilde,+}(s,a)  = p_{\wtilde,-}(s,a).
\end{align*}
%The reward and transition function on $M_{\wtilde,+}$ and $M_{\wtilde,-}$ coincide for actions not in $\mathcal C_\gamma(\wtilde)$. 
\paragraph{Batch algorithm does not have enough information}
\vspace{-0.3cm}
The above equation implies that the transitions and the rewards in the dataset could have originated from either $M_{\wtilde,+}$ or $M_{\wtilde,-}$.
In $s^\star$, the batch algorithm has two choices to determine the policy $\pihatstar_{\mathcal D}$ to return: 
choose action $a^\star$ and get a total return of $\frac{1}{2}$ or choose an action $a \neq a^\star$. The second choice  is $\frac{1}{2}$-suboptimal on $M_{\wtilde,-}$, while the first is at least $\frac{1}{2}$-suboptimal on $M_{\wtilde,+}$. At best, the batch algorithm can randomize between the two, showing the result.
\subsection{Proof Sketch of Theorem \ref{thm:BPI:ExponentialSeparation}}
It remains to exhibit an online algorithm that can solve this problem instance using $O(d)$ queries. The algorithm proceeds as follows: 1) it tries to locate the position of the hyperspherical cap by learning the vector $w$ and 2) it probes the hyperspherical cap to learn the $\pm$ sign of the MDP.

\paragraph{Identifying the position $\boldsymbol w$ of the hyperspherical cap}
Consider the following adaptive algorithm that submits policy-induced queries. The algorithm first plays the actions $\gamma e_1,\dots,\gamma e_d$ in $s^\star$ (these are $d$ policies that generate trajectories of length one where $\gamma e_i$ is the only action). %By construction, these actions are always outside the hyperspherical cap $\mathcal C_\gamma(w)$. 

Upon receiving the transition functions $p_w(s' = \gamma e_i \mid (s^\star,\gamma e_i))  = 
\min\{ \frac{1}{\gamma} (\gamma e_i)^\top w, 1 \} =  e_i^\top w $ for all $i \in [d]$, the agent can determine the $w$ vector (which identifies the hyperspherical cap $\mathcal C_\gamma(w)$) from the transition functions by solving a (non singular) linear system of equations. % associated with the MDP). %Then the agent probes the hyperspherical cap to gain knowledge of the reward function, which identifies the sign of the MDP.
%Precisely, upon playing $\gamma e_1,\dots,\gamma e_d$ in $s^\star$ 

\paragraph{Identifying the sign $\boldsymbol \pm$ of the MDP}
Next, the algorithm plays the state-action $(s^\star,w)$ to probe the hyperspherical cap  to observe the reward ($+1$ or $0$) which identifies the sign of the MDP. Since the MDP is now precisely identified, the agent can predict the value of any policy, and in particular, it can return the optimal policy.

\section{Conclusion}
This work presents exponential lower bounds for batch RL under very strong assumptions. In general, models are never correct, observations are noisy, and a batch algorithm needs to return an answer using whatever dataset is available; clearly the lower bounds continue to hold in these more general settings as much as they do when using more general predictors (like neural networks) which contain the linear setting as a special case. 

%This work quantifies the cost for adopting a purely batch approach for reinforcement learning with function approximation; in the worst case, such cost is exponential. Our hard instances can only arise in infinite horizon settings, showing exponential separation between finite and infinite horizon batch problems. 


Beyond the exponential lower bounds, an  important result of this work is that whenever function approximation is implemented, online exploration is required to achieve polynomial sample efficiency on certain problems. %, showing an exponential separation between batch and online RL. 
As these hard instances can only arise in infinite horizon settings, there exists an exponential separation between finite and infinite horizon batch problems. 

Finally, this work helps formalize some of the dangers of the deadly triad, which has long been known to cause algorithmic instabilities and divergence of dynamic programming algorithms. In a sense, the bootstrapping problem is for infinite horizon what the extrapolation problem is for finite horizon MDPs (and finite-steps algorithms), but unlike extrapolation, it cannot be mitigated by just adding more samples.

%\section*{Acknowledgment}
%The author is grateful to Emma Brunskill and Mykel Kochenderfer for providing useful  feedback on an earlier draft. The work was done while the author was visiting the Simons Institute for the Theory of Computing.

==> fig5.tex <==
\begin{tikzpicture}
\def\r{2.0};
\filldraw[color=gray!50, fill=gray!10] (0,0) -- (\r,0) arc (0:90:\r) -- (0,0) ;
\filldraw[darkgray!75] (0,0) circle (1pt) node[anchor=east] {$\vec 0$};
\draw[gray, fill=gray!50] ({\r*cos(30)},{sin(30)*\r}) arc(30:60:{\r}) -- cycle;
\draw[blue!75, ->] (0,0) -- node[near end, sloped, above] {\scriptsize $a_1$} ({\r*1/sqrt(10)},{\r*3/sqrt(10)});
\draw[darkgray!75, ->] (0,0) -- node[pos = 0.95, sloped, above] {\scriptsize $w$} ({\r*1.2/sqrt(2)},{\r*1.2/sqrt(2)});
\draw[blue!75, ->] (0,0) -- node[near end, sloped, below] {\scriptsize $a_2$} ({\r*3/sqrt(10)},{\r*1/sqrt(10)});
\end{tikzpicture}
